CONNA: Addressing Name Disambiguation on The Fly

Name disambiguation is a key and also a very tough problem in many online systems such as social search and academic search. Despite considerable research, a critical issue that has not been systematically studied is disambiguation on the fly -- to complete the disambiguation in the real-time. This is very challenging, as the disambiguation algorithm must be accurate, efficient, and error tolerance. In this paper, we propose a novel framework -- CONNA -- to train a matching component and a decision component jointly via reinforcement learning. The matching component is responsible for finding the top matched candidate for the given paper, and the decision component is responsible for deciding on assigning the top matched person or creating a new person. The two components are intertwined and can be bootstrapped via jointly training. Empirically, we evaluate CONNA on two name disambiguation datasets. Experimental results show that the proposed framework can achieve a 1.21%-19.84% improvement on F1-score using joint training of the matching and the decision components. The proposed CONNA has been successfully deployed on AMiner -- a large online academic search system.

==> data_observation.tex <==
\section{AMiner Data Observation}
\label{sec:Obser}

We collect the name disambiguation dataset from AMiner Billboard\footnote{https://www.aminer.cn/billboard}, which is a website publishing a variety of AMiner online real data benchmarks for data mining and data analysis. The dataset contains 800 common person names and  358,754 papers belonging to 12,484 persons.
Before presenting our model,  we have conducted an in-depth analysis of the AMiner dataset. And then, we did find some interesting phenomenon. 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.47\textwidth]{Figures/figure_author_dis}
	\caption{\label{fig:distri_author} Distribution of the number of co-occurrence authors.}
\end{figure}

Let us consider a simple baseline model - SVM to directly formalizes the continuous name disambiguation as a binary classification problem. Given a paper and some candidate authors, the SVM model firstly extracts several traditional interaction-features about the co-occurrence number of authors, the similarity of title, venue, and organizations between paper and each candidate author, then, SVM outputs the probability of the candidate author is the right author of the paper (predict to 1),  finally, we rank the candidate authors by their probability.
Follow the process, we systematically evaluate the SVM performance on the AMiner dataset. The evaluation metric is Hit Ratio@K (HR@K) which is the ranking metric measuring the percentage of the candidate lists
with the right person ranked before top K. At there, we empirically set K is 1 because we pay more attention to whether the top-ranked author is the right author or not. Unexpectedly, the SVM model achieves not bad HR@1 performance - 83.1\%, which confuses us that the continuous name disambiguation task is not very challenging? 
\begin{table}
	\centering
	\caption{\label{tb:Different_case_per} Different Case Performance (\%).}
	\begin{tabular}{cccc}
		\noalign{ \hrule height 1.2pt}
		\textbf{Case}  &  \textbf{\tabincell{c}{Easy Cases \\ (X $\geq$ 0.4)}}  & \textbf{\tabincell{c}{Hard Cases \\ (X $<$ 0.4)}}  & \textbf{Overall} \\
		\noalign{ \hrule height 1.2pt}
		\textbf{Data Ratio}  & \textbf{77.86} & 22.14 & ---     \\\hdashline
		\textbf{HR@1} &\textbf{90} & 64.6 & 83.1 \\
		\noalign{ \hrule height 1.2pt}
	\end{tabular}
\end{table}
Liu et al. \cite{liu2013s} researches a problem of linking users across multiple online communities which is similar to our task. In that paper \cite{liu2013s}, Liu et al. have made a survey based on the huge social network dataset, and then, he come to the conclusion that traditional username-related feature is important! Some instances can be done precisely by using only traditional username-related features.
Inspired by the conclusions in \cite{liu2013s}, we count the distribution of the co-occurrence number of authors of all paper-candidate author pairs on AMiner dataset. Fig. 2 presents the result. The X-axis is the proportion of the number of co-occurrence authors to all authors of the paper. A bigger ratio of the number of co-occurrence authors indicates the candidate author is more likely to be the right person of the paper, and also the instance is easy to distinguish and predict. The Y-axis is the data proportion. From the Fig. 2, we can see that the main part of instances has a bigger ratio of the number of co-occurrence authors. For the following analysis, we empirically set a line X = 0.4 to distinguish the instances whose ratio of the number of co-occurrence authors bigger than 0.4 which we called easy cases and those smaller than 0.4 which we called hard cases. Table. 1 demonstrate the accurate data ratio and performance in each case. From the Fig. 2, we can see that easy cases account for the majority part of the whole instances which is up to 77.86\%, and its Hit@1 performance is 90\% which is pretty good. While the hard cases occupy a small part which is about 22.12\%, and it has a poor Hit@1 performance - 64.6\%. Based on the observations, we comprehensively analyzing the continuous name disambiguation task on the real online scenario. And we can conclude that the task is very challenging and meaningful on the hard cases. Because superior paper assignment results is an important prerequisite ensuring the effectiveness of expertise search and personalized academic services.
In the experiment section, we will compare our proposed model with the baseline model on both the overall dataset and different cases data. 


